ROCK: Causal Inference Principles for Reasoning about Commonsense Causality

Commonsense causality reasoning (CCR) aims at identifying plausible causes and effects in natural language descriptions that are deemed reasonable by an average person. Although being of great academic and practical interest, this problem is still shadowed by the lack of a well-posed theoretical framework; existing work usually relies on deep language models wholeheartedly, and is potentially susceptible to confounding co-occurrences. Motivated by classical causal principles, we articulate the central question of CCR and draw parallels between human subjects in observational studies and natural languages to adopt CCR to the potential-outcomes framework, which is the first such attempt for commonsense tasks. We propose a novel framework, ROCK, to Reason O(A)bout Commonsense K(C)ausality, which utilizes temporal signals as incidental supervision, and balances confounding effects using temporal propensities that are analogous to propensity scores. The ROCK implementation is modular and zero-shot, and demonstrates good CCR capabilities.

==> sections/unused/notes.tex <==
%!TEX root = ../main.tex

\section{Notes}
\subsection{NAACL}

There are three papers on causality in the main conference, but none is about commonsense causality: one focused on document-level event causality identification (ECI), not using causal inference tools; one focused on document-level causal recovery for keywords; and one performed causal inference with textual data.
Causality in the last two papers is measured by the average treatment effect (ATE), which can be estimated using propensity score matching (PSM, a canonical method).

1. Graph Convolutional Networks for Event Causality Identiﬁcation with Rich Document-level Structures (link)

This paper studied the document-level event causality identification (ECI) problem --- predict the causal relationship between two event mentions of interest in a document. The causality here is not commonsense causality nor statistical causality; it is the regressand in this supervised learning problem.

In their graph model, nodes stand for event or entity mentions and edges their interactions. Six types of interactions (sentence boundary, coreference structure, mention span, context-based semantic, and knowledge-based semantic) are modeled, each associated with a score to be aggregated to form the weight of the edge. A graph convolutional neural net (GCN) is then applied. They test their method (called RichGCN) on EventStoryLine and Causal-TimeBank, which has better F1 scores than several baselines.

Comment: This paper provides a clever way of modeling edge weights using discourse, syntax, and semantic information in a graph, though I feel "causality" here is nothing more special than labels in datasets.

2. Everything Has a Cause: Leveraging Causal Inference in Legal Text Analysis (link)

This paper proposed a graph-based causal inference (GCI) framework, focusing on reasoning causality of keywords from fact descriptions of legal documents such as criminal cases.
In their framework, each node in the causal graph corresponds to (a cluster of similar) keywords extracted from legal documents. Causality is assessed in two steps: (i) Greedy fast causal inference (GFCI) is performed for causal discovery on this graph, identifying edges of influence. (ii) PSM was used to estimate ATE between nodes. 

This paper also discusses potential ways of imposing causal signals into neural nets by (i) adding an MSE loss between the weight of the attention layer and the estimated ATE (Fig. 3) and (ii) applying LSTM to causal chains (extracted from the causal graph). 

Comment: Built on top of existing tools from causal inference, this paper shows how to use it to reason causal relationships of some document-level tokens (legal keywords) and potential ways of imposing causal signals in neural nets.

3. Causal Effects of Linguistic Properties (link)

This paper is about causal inference on textual data where they studied if linguistic properties (treatments, e.g., if the text has a positive or negative sentiment) of texts (e.g., Amazon reviews) causes some responses (e.g., whether the product link is clicked), adjusting for confounding effects (e.g., the text itself and other confounders such as the type of the product).
Since the linguistic properties are not always observed, proxy labels are used (e.g., predictions from some models). Interestingly, a model was trained to adjust the confounding effect from the texts, and the ATE is then estimated in a plug-in manner.

They showed that on the Amazon review dataset under artificially constructed noisy proxy labels, their method (TextCause) is more accurate on average. They also argued it is helpful to adjust for texts instead of only using the (proxy) labels by showing some cases where predictions of their method deviates largely from the ground truth, which I find less convincing.

Comment: This paper contains some math as they proved some causal inference flavored results. Although interesting, I think some arguments are lacking (e.g., on why it is necessary to adjust for texts), and the dataset they tested is somewhat artificial.

\subsection{ACL}
Event Causality
==========================================================
Learning Faithful Representations of Causal Graphs
Ananth Balashankar, Lakshminarayanan Subramanian
Paper: https://aclanthology.org/2021.acl-long.69
Talk: https://underline.io/lecture/25432-learning-faithful-representations-of-causal-graphs
This paper proposed a fine-tuning method for approximate non-document-level event causality by a similarity-like measure that minimizes violations of a notion of the faithfulness of causality of events. In particular, their algorithm computes the strength of causal link of **known** causal graphs where nodes are events.  
Pros:
+ Fine-tuning making use of Heindorf’s CauseNet knowledge base.
+ Making use of a (based on known results) faithful score in fine-tuning.
Cons:
- Needs causal graphs to be known, which in their case is human-annotated.
- The main result (Table 3) is only on Yahoo! QA dataset, with no results on generalization.
==========================================================
Doing Good or Doing Right? Exploring the Weakness of Commonsense Causal Reasoning Models
Mingyue Han, Yinglin Wang
Paper: https://aclanthology.org/2021.acl-short.20
TLDR: the COPA dataset used in evaluating commonsense causality models contain biases.
This paper studies semantic-similarity biases and claimed to identify two vulnerability of the COPA dataset through (i) perturbation by distractors, such as a third choice; (ii) masking question type, such as from “cause” to “effect.” They show that the pretrained LM-based models suffer from these vulnerabilities and proposed to mitigate them by regularizing the square distance between the logits of the model outputs from two plausible options. They show this method is more robust when evaluated on BCOPA-CE, an extended dataset created by flipping the cause/effect of the samples in COPA.
Pros:
+ Identify vulnerabilities, corroborating Kavumba 2019.
+ Propose a regularization method that they claim to mitigate the vulnerabilities identified.
Cons: 
- Model/architecture choice seems restrictive, not using SOTA methods and no real causal inference.
- Masking question type seems not to be a vulnerability: a good causal model should be able to deal with that.
- Their extension from COPA to BCOPA-CE is somewhat trivial.
- Needs fine-tuning, not a zero-shot method.
==========================================================
ExCAR: Event Graph Knowledge Enhanced Explainable Causal
Li Du, Xiao Ding, Kai Xiong, Ting Liu, Bing Qin
Paper: https://aclanthology.org/2021.acl-long.183/
Talk: https://underline.io/lecture/6378-knowledge-enhanced-natural-language-inference-based-on-knowledge-graphs
This paper proposed a framework called ExCAR to reason event causality based on existing graph knowledge bases. It first retrieves causal event graph using a pretrained ELMo and identify events chains by DFS from the cause event to the effect event. BERT embedding is then used to encode events in the chain. A learnable one-layer NN is used to estimate the conditional probability of an edge given its predecessors, which they call causal strength. The causal strength of a chain is then defined as the product of these conditional probabilities in the chain. Finally, logistic regression is used to predict the aggregated causal score from those in each chain.
 Pros
 + Use an external knowledge graph for causal reasoning by estimating causal strengths along event chains.
 + Considers “antecedents” and superimposed causal effect (causal strength between events change due to context change), which is analogous to the “context” in our previous discussions.
 Cons
 - The construction of causal score is a bit arbitrary and artificial: it does not explicitly adjust for confounders; the product of conditional probabilities (Eq. 7) needs further assumptions for their validity.
 - Need fine-tuning to learn the parameters, not zero-shot.
 - Experiments were only done on COPA, with no generalization results. Results could also suffer from COPA’s own limitations as pointed out by the other paper.
 - Performance is not better than SOTA (which they did not compare).
 - Code is unavailable yet.
==========================================================
The following three papers
(A) Improving Event Causality Identification via self-supervised Representation Learning on External Causal Statement
Paper: https://aclanthology.org/2021.findings-acl.190/
Talk: https://underline.io/lecture/26281-improving-event-causality-identification-via-self-supervised-representation-learning-on-external-causal-statement
(B) Knowledge-Enriched Event Causality Identification via Latent Structure Induction Networks
(also discussed by Rotem)
Paper: https://aclanthology.org/2021.acl-long.376.pdf
Talk: https://underline.io/lecture/25698-knowledge-enriched-event-causality-identification-via-latent-structure-induction-networks
(C) LearnDA: Learnable Knowledge-Guided Data Augmentation for Event Causality Identification
Paper: https://www.aclanthology.org/2021.acl-long.276
Talk: https://underline.io/lecture/25618-learnda-learnable-knowledge-guided-data-augmentation-for-event-causality-identification
are by the same authors modulo permutation: Xinyu Zuo, Pengfei Cao, Yubo Chen, Kang Liu, Jun Zhao, Weihua Peng, Yuguang Chen.
They proposed frameworks for event causality identification (ECI) that makes use of different external knowledge by designing different modules and evaluate on the EventStoryLine and Causal-TimeBank datasets. In particular,
(A) called it CauSeRl and uses external causal statements from GLUCOSE, ATOMIc, and DISTANT;
(B) called it LSIN and uses descriptive knowledge from graph KB ConceptNet and COMET;
(C) called it LearnDA and uses WordNet, VerbNet, FrameNet+PDTB2 to extract event pairs for data augmentation.
They report that F1 scores of their methods are about 1%-2% higher than previous baselines while the performances of (A) (B) (C) are *very* similar, with the F1-score being (A) < (B) < (C).
==========================================================
Some other papers making using causal inference
==========================================================
Discovering Topics in Long-tailed Corpora with Causal Intervention
Xiaobao Wu, Chunping Li, Yishu Miao
Paper: https://aclanthology.org/2021.findings-acl.15
As corpora in the real world are naturally long-tailed (Cf. Zipf’s law), this paper proposed to use a causal inference framework to explain and overcome the issues of topic modeling on long-tailed corpora. A new model, deconfounded topic model (DecTM), is introduced and shown can mitigate the long-tail bias, producing more diverse topics and better disclose the semantics of documents about tail topics.
==========================================================
Causal Analysis of Syntactic Agreement Mechanisms in Neural Language Models
Matthew Finlayson, Aaron Mueller, Sebastian Gehrmann, Stuart Shieber, Tal Linzen, Yonatan Belinkov
Paper: https://aclanthology.org/2021.acl-long.144/
This paper applies causal mediation analysis to pre-trained LMs by viewing the LM as a causal graph and intermediate components (such as a neuron) as mediators to investigate model’s preferences for grammatical inflections and S-V agreements.
Interesting findings includes: for certain LM such as GPT2, it is always easier to form agreement dependencies between verbs and plural subjects than singular ones.

% \subsection{Discussions and TODOs}

% \paragraph{TODO}
% \bitem
%     \item Define causal strength from scores on three edges 
%     ($\cau_{C\to E}$, $\Exp_T\cau_{T\to C}$, $\Exp_T\cau_{T\to E}$).
%     \item Identify "causally equivalent classes" of events to form "event clouds".
% \eitem 

% \subsection{Can we assess the strength via counter-factuals?}
% \jiayao{This is a previous idea, not on the path in our recent discussions.}

%     We are given two events \red{$C$} and \blue{$E$}, let $T$ be the binary variable
%     that indicate whether $C$ temporally precedes $E$.
    
%     \beg \red{Alice feels hungry} \textbf{then} \blue{she enters a restaurant}.
%     \eeg
    
%     In the causal line of reasoning, we analogously wants to study the
%     effect on \blue{$E$} due to \red{$C$} under the confounding temporal
%     information $T$. Substituing into the DoE framework, the above
%     example becomes:
%     \bitem
%         \item Deleting the edge $C\to E$: an ``experiment''
%             where \emph{one} \blue{enters a restaurant} regardless
%             \red{whether she feels hungry} and regardless of the temporal relation.
%         \item $\Pr_{C\to E}(e\vert c, t)
%             = \Pr_{C\to E}(e \vert t)
%             = \sum_{c'} p(e \vert t, c') p(x')$:
%                 ``conditional probability'' of \blue{entering the restaurant}, given \red{$C$} happens before \blue{$E$}
%                 but with \emph{random} events $C$.
%     \eitem 
%     In this case $\cau_{C \to E}$ measures the impact
%     of destroying the coupling between \red{Alice feels hungry}
%     and \blue{she enters a restaurant}. We consider two cases:
%     \bitem
%         \item $\cau_{C\to E} \approx 0$ means $\Pr_{C\to E}(e\vert c,t)$ and
%         $\Pr(c,e,t)$ are very close, thus we do \emph{note} expect
%         there to be any causal effects from $C$ to $E$
%         \item $\cau_{C\to E} \gg 0$ means the destruction of edge
%         has great impact, thus the causal link $C\to E$ is significant.
%     \eitem 
    
%     Algorithmically, given a knowledge base $f: (C,E,T) \to \sR_+$ that
%     output a confidence score of \red{$C$} and \blue{$E$} has
%     temporal order $T$, we define the causal strength as
%     \ba
%         \cau_{c\to e}
%         = f(c,e,t) \log \frac{
%             f(e\vert t, c)
%         }{\sum_{c' \distas \mathcal{C}} 
%             f(e\vert t, c') f(c')
%         },
%     \ea
%     where we estimate the conditional as
%     \ba
%         f(e|t,c) = 
%         \frac{
%                 \sum_{e' \distas  \mathcal{E}: e' \asymp e} f(c, e', t)
%             }{
%                 \sum_{e' \distas  \mathcal{E}} f(c, e', t)
%             },
%     \ea
%     and write $e' \asymp e$ if $e$ and $e'$ are equivalent.
    
% \subsection{Preliminary result on COPA using only $\cau_{C\to E}$}

%     In order to compute the causal strength
%     of a given event pair $(c,e)$, we follow
%     the following:
%     \bitem
%         \item Filter all events $T=\{t: t \le c \le e\}$  using
%         TemProb knowledge base.
%         \item For each $t \in T$, estimate
%         \ba
%             f(e \vert t,c)
%             = \frac{
%                 \sum_{e'\in \calE : e'\asymp e} f(c, e', t)
%             }{
%                 \sum_{e'\in \calE} f(c, e', t)
%             },
%         \ea
%         the conditional probability of event $e$ happens after $t$ and $c$,
%         where the set $\calE$ is sampled from the KB such that
%         \ba
%             \calE = \{e' : t \le c \le e'\},
%         \ea
%         and $e' \asymp e$ means $e$ and $e'$ are causally-similar, where
%         we can filter based on the contextual score, such as one given by
%         the GloVe similarity. We set $e' \asymp e$ if their GloVe score
%         is larger than $0.5$.
        
%         \item Estimate 
%         \ba
%             \cau_{c \to e}
%             = \sum_{t \in \calT}    
%                 f(c,e,t) \log \frac{
%                     f(e \vert t,c )
%                 }{
%                     \sum_{c' \in \calC} f(e \vert t, c') f(c')
%                 }
%         \ea
        
%     \eitem
    
    
    

==> sections/unused/old_notes.tex <==
\section{Old Section 2}
    We will use capital letters such as $T, C, E$ to denote
    generic events, and lowercase letters such as $t,c,e$ to denote
    specific event instances. Events can be represented by verbs or other structures.
    We will overload $<$ and $>$ on events to denote temporal order.
    and use $f(a_1, a_2,\ldots )$ to denote a score function that assigns a
    probability
    \ba
        f(a_1, a_2, \ldots, a_k) \coloneqq \Pr(a_1 < a_2 < \cdots < a_k)
    \ea
    for events $a_1$ occurs before $a_2$, which occurs before $a_3$, etc.
    In the simplest case, this can be thought as an query to the TemProb
    knowledge base yet this abstraction allows us to cluster events
    based on context, as is motivated in the following.

    A critical view we shall undertake is to identify an event $E$ as
    a representative from a ``causally-equivalent'' class of events, which
    we shall denote by $\calE(E)$. An observed
    event $e$ is thus viewed generated by some underlying sampling distribution
    which we shall assume to be uniform over $\calE(e)$.
    For ease of exposition, we will use $e$ and $\calE(e)$ interchangably.

    Thus our framework for evaluating the causal strength is summarized as follows:
    \benum
        \item Given observed events $c_0$ and $e_0$, we are asked to evaluate
        the causal strength from $c_0$ to $e_0$ (how likely does the event
        $c_0$ cause the event $e_0$?)
        \item Identify the equivalent classes $\calE(c_0)$ and $\calE(e_0)$.
        \item Construct causal graphical model to adjust for temporal confounders.
        \item Output the causal score of $c_0\to e_0$.
    \eenum
    In the next subsections, we will introduce the type of confounding variables
    considered in this paper, the corresponding causal graphical model,
    and how we identify equivalent classes based on temporal knowledge.
    \jiayao{
        The goal is to locate a potential confounder. The following the confounder
        is an event. It might also be possible to view it as, for example, a
        temporal variable. This path is not taken but the notes are in the appendix.
    }

    \benum
        \item Sampling events $T$ (TemProb , ASER (co-occurence))
        \item Using another LM to predict edge weights (MASK, CoCoLM)
        \item Estimate causality score.
    \eenum

\subsection{Adjusting for Temporal Confounding Events}
    Given two events $C$ and $E$ with $C<E$, when does $C$ not cause $E$?
    A plausible scenario is when there exists some event $T$ (or more general, a
    sequence of such events) with $T < C$ that may have caused $E$ (which
    may or may not cause $C$).
\begin{figure*}
    \centering
	 \begin{subfigure}[t]{0.5\linewidth}
	    \centering
	    \resizebox{\linewidth}{!}{\input{./figs/graph/single_t.tikz}}
	    \caption{Graphical model for a single event $T$.} \label{fig:casaulgraph:single}
	\end{subfigure}%
    \begin{subfigure}[t]{0.5\linewidth}
        \resizebox{\linewidth}{!}{\input{./figs/graph/multi_t.tikz}}
	    \caption{Graphical model for multiple events $T_i$.} \label{fig:casaulgraph:multi}
	\end{subfigure}%
        \caption{\textbf{Graphical model for modelling causality between events.}}
        \label{fig:casaulgraph}
\end{figure*}
    Indeed, if we are able to group similar events together, it suffices
    to group all $T_i$'s into a singl event cloud $T$, which is illustrated
    in \Cref{fig:casaulgraph}.

    To assess the causality strength between observed events $c_0$ and $e_0$,
    $\cau_{c_0\to e_0}$, we adapt the cutting-wire formulation in \cite{janzing2013quantify}.
    We view those observed events as representatives of equivalent classes of events that
    is generated by sampling uniformly at random.
    to compute the KL divergence between the original
    distribution $p(c, e,t)$ and the intervention distribution $p(c',e,t)$
    with $c'$ being and independent copy of $c$ while keeping the marginal
    distribution on $e$ and $t$ unchanged.

    We will model $T$ as a random event that happen before $c_0$ and $e_0$
    whose sampling distribution is defined as $p_T(t)$ supported on $\calT$.
    \ba
        \cau_{c_0\to e_0}
        =
        \frac{1}{\abs{\calT}} \sum_{t \in \calT}
            f(t, c_0, e_0) \log \frac{
                p(e_0 \vert t, c_0) }{
                \Exp_{c'\distas P_{c_0}} p(e_0 \vert t, c')
            }, \quad
         \Exp_{c'\distas P_{c_0}} p(e_0 \vert t, c')
         = \frac{1}{\abs{\calC}} \sum_{c' \in \calC} p(e_0\vert t, c').
    \ea
    where we write $\calC$ for the support of $P_{c_0}$, the sampling
    distribution of $c_0$.
    % \jiayao{
    %     I think it makes more sense to sample $c'$ from the subset $\calC'(t)\subset\calC$
    %     that contains events in $\calC$ that are temporally after $t$.
    %     I will try to introduce r.v.s that corresponding to temporal orders.
    % }
    In the above display, the conditional probabilities are computed as
    \ba
        p(b_1 \vert a_1, a_2, a_1 < a_2) = \frac{ f(a_1, a_2, b_1) }{
            \sum_{b: b > a_1, b > a_2} f(a_1, a_2, b)
        } = \frac{ f(a_1, b_1) f(a_2, b_1) }{
            \sum_{b: b > a_1, b > a_2} f(a_1, b) f(a_2, b)
        }.
    \ea

    To compute the term
    \ba
    \frac{
            p(e_0 \vert t, c_0) }{
            \Exp_{c'\distas P_{c_0}} p(e_0 \vert t, c')
        },
    \ea
    it is important to specify $P_{c_0}$. There are
    three ways:
    \benum
        \item Sampling events that temporally
        after $t$ and before $e$.
        \item $P_{c_0}$ consists of $c_0$ and the
        negation of $c_0$.
        \item Paraphrasing $c_0$.
        \item Sampling $P_{c_0}$ using text entailment.
        Treat entailment as an equivalent class of $c_0$.
    \eenum

    Similarly, we can compute
    \ba
        \cau_{t\to e_0} &= \sum_{t, c_0, e_0}
            f(t, c_0, e_0) \log \frac{p(e_0 \vert t, c_0)}
                {
                \Exp_{t' \distas P_{t}} p(e_0\vert t', c_0)
                % \sum_{t'} p(e_0 \vert t' c_0, ) p(t')
                }, \\
        \cau_{t\to c_0} &=
            \sum_{t, c_0, e_0} f(t, c_0, e_0)
                \log \frac{p(c_0 \vert t)}{
                \Exp_{t' \distas P_t} p(c_0\vert t')
                %\sum_{t'} p(x\vert t')p(t')
                },
    \ea
    or algorithmically,
    \ba
        \Exp\cau_{t\to e_0} &= \frac{1}{\abs{\calT}} \sum_{t\in \calT}
            f(t, c_0, e_0) \log \frac{p(e_0 \vert t, c_0)}
                {
                 \frac{1}{\abs{\calT}} \sum_{t'\in\calT} p(e_0\vert t', c_0)
                }, \\
        \Exp\cau_{t\to c_0}
        &= \frac{1}{\abs{\calT}} \sum_{t\in \calT}
            f(t, c_0, e_0)  \log \frac{p(e_0 \vert t, c_0)}
            {\frac{1}{\abs{\calT}} \sum_{t'\in\calT} p(e_0\vert t', c_0)}.
    \ea


    There might be two ways henceforth:
    \bitem
        \item Compute $\cau_{c_0\to e_0}$, $\Exp_{t\distas P_T} \cau_{t \to e_0}$,
        and $\Exp_{t\distas P_T} \cau_{t\to c_0}$, that enables us to evaluate
        the effect of removing the edge $c_0\to e_0$, $t\to e_0$, and $t\to c_0$
        respectively. Then construct a metric based on these three values that instantiates the intuition that ``$c_0$ causes $e_0$ if the link
        $c_0\to e_0$ is stronger than $t \to c_0$ and $t \to e_0$ combined.''
        Here we will need to randomize over $t$ as it is not observed.

        \item If we are only interested in selecting the best answer among a
        set of plausible choices (e.g., scenario under COPA task), we may
        be able to directly compare the values $\cau_{c_0 \to e_0}$
        and $\cau_{c_1 \to e_0}$ to reason which one of $c_0$ and $c_1$
        is more likely to cause $e_0$.

    \eitem

    An aggregated score for the causal strength of $c_0\to e_0$
    may be defined in terms of the causal strengths on each of the edge.
    % \ba
    %     w(c_0\to e_0) =
    % \ea

    \subsection{Implicit Events}
        A more elaborated causal model would also
        encompasses implicit events, i.e., an event
        that occurred ($D$) but not mentioned in the text.


    \subsection{Construction of Event Clouds}
        The key to our framework for event causality is to identify sets
        of events that can be viewed as  ``causally equivalent classes'',
        or ``event clouds.''

        \jiayao{
            One way is to use LMs incorporated with TemProb knowledge?
        }






% \subsection{Can we assess the strength via counter-factuals?}
% \jiayao{This is a previous idea, not on the path in our recent discussions.}

%     We are given two events \red{$C$} and \blue{$E$}, let $T$ be the binary variable
%     that indicate whether $C$ temporally precedes $E$.

%     \beg \red{Alice feels hungry} \textbf{then} \blue{she enters a restaurant}.
%     \eeg

%     In the causal line of reasoning, we analogously wants to study the
%     effect on \blue{$E$} due to \red{$C$} under the confounding temporal
%     information $T$. Substituing into the DoE framework, the above
%     example becomes:
%     \bitem
%         \item Deleting the edge $C\to E$: an ``experiment''
%             where \emph{one} \blue{enters a restaurant} regardless
%             \red{whether she feels hungry} and regardless of the temporal relation.
%         \item $\Pr_{C\to E}(e\vert c, t)
%             = \Pr_{C\to E}(e \vert t)
%             = \sum_{c'} p(e \vert t, c') p(x')$:
%                 ``conditional probability'' of \blue{entering the restaurant}, given \red{$C$} happens before \blue{$E$}
%                 but with \emph{random} events $C$.
%     \eitem
%     In this case $\cau_{C \to E}$ measures the impact
%     of destroying the coupling between \red{Alice feels hungry}
%     and \blue{she enters a restaurant}. We consider two cases:
%     \bitem
%         \item $\cau_{C\to E} \approx 0$ means $\Pr_{C\to E}(e\vert c,t)$ and
%         $\Pr(c,e,t)$ are very close, thus we do \emph{note} expect
%         there to be any causal effects from $C$ to $E$
%         \item $\cau_{C\to E} \gg 0$ means the destruction of edge
%         has great impact, thus the causal link $C\to E$ is significant.
%     \eitem

%     Algorithmically, given a knowledge base $f: (C,E,T) \to \sR_+$ that
%     output a confidence score of \red{$C$} and \blue{$E$} has
%     temporal order $T$, we define the causal strength as
%     \ba
%         \cau_{c\to e}
%         = f(c,e,t) \log \frac{
%             f(e\vert t, c)
%         }{\sum_{c' \distas \mathcal{C}}
%             f(e\vert t, c') f(c')
%         },
%     \ea
%     where we estimate the conditional as
%     \ba
%         f(e|t,c) =
%         \frac{
%                 \sum_{e' \distas  \mathcal{E}: e' \asymp e} f(c, e', t)
%             }{
%                 \sum_{e' \distas  \mathcal{E}} f(c, e', t)
%             },
%     \ea
%     and write $e' \asymp e$ if $e$ and $e'$ are synomous events.


% \subsection{Constructing the Event Graph}
%     Given two events $C$ and $E$, we wish to
%     \bitem
%         \item Construct a sequence of events $\{T_i\}_{i=1}^m$
%         such that their temporal order
%     \eitem

% \subsection{Data Structure for TemProb}
%     In order to compute the causal strength
%     of a given event pair $(c,e)$, we follow
%     the following:
%     \bitem
%         \item Filter all events $T=\{t: t \le c \le e\}$
%         from the KB.
%         \item For each $t \in T$, estimate
%         \ba
%             f(e \vert t,c)
%             = \frac{
%                 \sum_{e'\in \calE : e'\asymp e} f(c, e', t)
%             }{
%                 \sum_{e'\in \calE} f(c, e', t)
%             },
%         \ea
%         the conditional probability of event $e$ happens after $t$ and $c$,
%         where the set $\calE$ is sampled from the KB such that
%         \ba
%             \calE = \{e' : t \le c \le e'\},
%         \ea
%         and $e' \asymp e$ means $e$ and $e'$ are causally-similar, where
%         we can filter based on the contextual score, such as one given by
%         the GloVe similarity.

%         \item
%         \ba
%             \cau_{c \to e}
%             = \sum_{t \in \calT}
%                 f(c,e,t) \log \frac{
%                     f(e \vert t,c )
%                 }{
%                     \sum_{c' \in \calC} f(e \vert t, c') f(c')
%                 }
%         \ea

%


==> sections/unused/problem.tex <==
%!TEX root = ../main.tex
\newcommand{\evts}{E}
\newcommand{\evtsets}{\calE}
\newcommand{\metric}{\operatorname{m}}

\section{A Mathematical Framework for Reasoning Commonsense Causality}
\subsection{Setup and Notation}

    We use lowercase letters such as $e_1, e_2$ to denote events extracted from
    sentences in natural languages, which we represent as $3$-tuples consisting
    of the VERB, ARG0, and ARG1. We use capital letters to denote the indicator
    variable on whether an event happens, e.g., $Y = \ind{e_2 \text{ happens}}$.
    For notation consistency, we reserve symbols $X, D, Y$ for confounding,
    treatment and outcome events respectively, and their lowercase counterparts
    for their specific instantiations.
    Here the underlying probability space can be taken as the space encompassing
    all events in natural languages whose empirical version can be inferred from
    corpses.
    Given two events $e_1$ and $e_2$ as inputs, our goal is to reason,
    how strong (or weak) can we say there is a causal relationship from $e_1$
    to $e_2$, or  \emph{does $e_1$ causes $e_2$}? Clearly, the answer to this
    question depends on the \emph{context} which we denote by $C$.

    For our purpose, we mainly leverage temporal signal as the context based
    on the following observation:
    \begin{center}
	\emph{An event $e_2$ cannot be the cause for $e_1$ if $e_2$ happens temporarily after
	the event $e_1$}.
    \end{center}
    The converse of this statement is in general not true, however, for the
    simple reason that there might be unknown \emph{confounding} events
    $X$ that happens temporarily before both $e_1$ and $e_2$ that serves as
    the real cause, while the relationship between $e_1$ and $e_2$ is no
    more complicated than an innocuous association.
    In causal language, we model this confounding effect via
    the graph model given in \Cref{fig:casaulgraph}, where $X$
    is the indicator of confounding events.

    As Don Rubin pointed out, ``no causation without manipulation'',
    our model indeed fits in the realm of classical causal inference in that
    we can easily imagine a distribution on events in which we \emph{manipulate}
    the treatment event $X$ while keeping the confounding events $X$ fixed.
    \begin{figure*}
    \centering
	 \begin{subfigure}[t]{0.5\linewidth}
	    \centering
	    \resizebox{\linewidth}{!}{\input{./figs/graph/single_t.tikz}}
	\end{subfigure}%
	%\begin{subfigure}[t]{0.5\linewidth}
        %\resizebox{\linewidth}{!}{\input{./figs/graph/multi_t.tikz}}
	%    \caption{Graphical model for multiple  ,b events $T_i$.} \label{fig:casaulgraph:multi}
	%\end{subfigure}%
        \caption{\textbf{Graphical model for modeling causality between events.} Here $X$, $D$, and $Y$ models
	the confounding, treatment, and outcome events, respectively.}
        \label{fig:casaulgraph}
    \end{figure*}

    In our setup, the treatment variable would be the presence or absence
    of the given event $e_1$, the outcome being the other event $e_2$.
    The manipulation of the events

    We devise the following framework to reason commonsense causality based on our graphical model that
    contains four components.
    \paragraph{Event sampler.} Given an event $e$, the sampler $h : \evts \to \evtsets$ samples
	    a set of events that likely co-occur with $e$.

    \textbf{Predictor.} Given two events, the predictor $f: \evts \times \evts \to [0,1]$
	    computes $f(e_1, e_2) = \Pr(e_1 \text{ happens before } e_2)$.

    \textbf{Counterfactual generator.} Given an event $e$, the counterfactual generator $g : \evts \to \evtsets$
	    generate a set of events that are semantically interventions to the event $e$.

    \textbf{Scoring metric.} Given two events $e_1$ and $e_2$, the event sampler $h$,
	    predictor $f$, and the counterfactual generator $g$, the scoring function computes
	    a score $\metric(e_1,e_2; h, f, g)$ characterizes the causal strength from $e_1$ to $e)2$.

    We next describe how these four components are being designed.

    \subsection{Temporal-Aware LM Head}
	Toward the first step of constructing the event sampler or the predictor lies
	the central question on how to train a language model to be \emph{temporally aware},
	that is, being able to predict temporal probabilities of two given input events.
	To this end, we adapt the masked language modeling to fine-tune pre-trained language
	models on temporal event-pairs extracted from the New York Times articles spanning 20 years.
	Given two events $e_1$ and $e_2$, we add a mask between them and ask the LM to predict
	the token. We use the scores for the token ``before'' and ``after'' for the unnormalized
	probabilities that $e_1$ happens before (resp. after) $e_2$.

    \subsection{Causal Score}
	The core of our framework lies on the metric that quantifies causality.
	We discuss several options of such scores in this section. To this end,
	we need to be crystally clear about the units of the ``experiments'',
	what does ``manipulation'' mean in this context, and what pre-treatment
	variables are. Unlike classical causal inference which is usually performed
	on observational studies, the unique feature of language modeling allows
	us to \emph{impute} data using language models. In the causal inference spirit,
	if we want to investigate whether there is a causal link between the treatment
	variable $d_0$ and the outcome $y_0$, we can impute interventions of the treatment
	$\calD = \{d_i\}_{i=1}^n$, their corresponding outcome $\calY = \{y_i\}_{i=1}^n$. With a set
	of confounding events identified $\{x_i\}_{i=1}^m$, we can match a subset $\calD'$ of interventions in
	$\calD$ such that they are similar to $d_0$ in the sense that they have comparable
	pre-treatments. The change of the outcome $y$ due to intervention can then be understood as a measure
	for the causal strength that is analogous to the \emph{average treatment effect (on the treated)}
	in causal inference.

	Building on this identification, it is natural to measure the change of outcome by the
	change of the temporal probability of the intervention to the event $y_0$, which can be
	imputed by the predictor.
	
	\subsubsection{Baseline Temporal Score}
	    Perhaps that most straightforward baseline is to compute the change of temporal likelihood
	    due to confounders:
	    \ba
	    \,& \metric_n(d_0, y_0; h, f, g) \\ =&f(d_0, y_0) - \frac{1}{\abs{h(d_0)}} 
		\sum_{\substack{x \in h(d_0) \\ f(x, d_0) > 1-\eps}} f(x, y_0),
	    \ea
	    where $h(d_0)$ is the sampled events based on $d_0$; $f(x, d_0) > 1-\eps$ is used to filter all events
	    that have a relatively high probability to precede $d_0$ for some pre-determined $\eps > 0$.

	\subsubsection{AATE}
	    One of the working horse of causal inference is the matching method \red{cite}. Intuitively,
	    we want to find interventions that share comparable pre-treatments as the treatment.
	    In our setup, the pre-treatments are $h(d_0)$ and we can identify a matched subset $\calD'$
	    with
	    \ba
		\calD' := \left\{d\in\calD: \dist(d_0, d; h(d_0)) < \delta\right\},
	    \ea
	    where $\delta$ is a pre-determined confidence parameter and we set
	    \ba
		\,&\dist(d_0,d;h(d_0))\\
		=& \norm{ (f(x,d_0))_{x\in h(d_0)} - (f(x,d))_{x\in h(d_0)} }_p
	    \ea
	    for a suitable choice of $p$. Note that we write $(f(x,d_0))_{x\in h(d_0)}$ for
	    a $\abs{h(d_0)}$-dimensional vector. Once the matching is completed
	    we estimate the AATE via
	    \ba
	    \textsc{AATE} = 
	    f(d_0, y_0) - \frac{1}{\abs{\calD'}}
	        \sum_{d \in \calD'} f(d, y_0).
	    \ea


==> tables/A03_dataset_eg.tex <==
\begin{table*}
    \centering
    \resizebox{\linewidth}{!}{%
        \begin{tabular}{lll}
        \toprule
        Dataset & $C$ & $E$ \\
        \midrule
    \textsc{Copa} & \texttt{The player caught the ball.} &%
            \texttt{Her teammate threw it to her.} \\
    \textsc{Copa} & \texttt{The player caught the ball.} &% 
            \texttt{Her opponent tried to intercept it.} \\
    \textsc{PDTB3} &%
        \texttt{Some criminal lawyers speculated that the IRS was sending the letters} & \texttt{to test the issue} \\
    \textsc{PDTB3} &%
        \texttt{Mr. van Dover said the AT\&T team created the desired crystal changes by} & \texttt{bombarding superconductor samples with neutrons} \\
    \textsc{GLUCOSE} &% 
        \texttt{Gage wants safety} & \texttt{Gage turned his bike} \\
    \textsc{GLUCOSE} &%
        \texttt{Gage was close to a car} & \texttt{Gage turned his bike away from the car} \\
        \bottomrule
        \end{tabular}
    }
    \caption{\textbf{Examples of dataset considered in this paper,} 
        COPA (\cite{COPA}), PDTB3 (\cite{PDTB3}), and GLUCOSE (\cite{GLUCOSE}).}
    \label{tab:dataset:eg}
\end{table*}

